Gel'fand triples and boundaries of infinite networks

We study the boundary theory of a connected weighted graph $G$ from the viewpoint of stochastic integration. For the Hilbert space \HE of Dirichlet-finite functions on $G$, we construct a Gel'fand triple $S \ci {\mathcal H}_{\mathcal E} \ci S'$. This yields a probability measure $\mathbb{P}$ on $S'$ and an isometric embedding of ${\mathcal H}_{\mathcal E}$ into $L^2(S',\mathbb{P})$, and hence gives a concrete representation of the boundary as a certain class of "distributions" in $S'$. In a previous paper, we proved a discrete Gauss-Green identity for infinite networks which produces a boundary representation for harmonic functions of finite energy, given as a certain limit. In this paper, we use techniques from stochastic integration to make the boundary $\operatorname{bd}G$ precise as a measure space, and obtain a boundary integral representation as an integral over $S'$.

==> paths.tex <==
%%!TEX root = bdG.tex

\subsection{The boundary as equivalence classes of paths}
\label{sec:bdG-as-equivalence-classes-of-paths}

We are finally able to give a concrete representation of elements of the boundary. We continue to use the measure \quotprob from Theorem~\ref{thm:HE-isom-to-L2(S',P)}. %induced on the quotient $\Squoth $ as in Definition~\ref{def:quotprob}.  
Recall the Fock space representation of $L^2(\Schw',\prob)$ discussed in Remark~\ref{rem:Wiener-improves-Minlos}:
% if one were to reprove Theorem~\ref{thm:HE-isom-to-L2(S',P)} for $\sW$ defined only on \Harm, then \eqref{eqn:Minlos-expectation-integral} implies that we have a corresponding Fock space representation for the quotient:    
  \linenopax
  \begin{align}\label{eqn:Fock-repn-of-L2(S',P)-as-HE}
    L^2\left(\Squot,\quotprob\right) \cong \bigoplus_{n=0}^\iy \HE^{\otimes n}.
  \end{align}
  where $\HE^{\otimes 0} := \bC \one$ for a unit ``vacuum'' vector \one corresponding to the constant function, and $\HE^{\otimes n}$ denotes the $n$-fold \emph{symmetric} tensor product of \HE with itself. Observe that \one is orthogonal to \Fin and \Harm, but is not the zero element of $L^2(\Squoth,\quotprob)$.
  
\begin{lemma}\label{thm:int(u)=0-over-bdG}
  For all $v \in \Harm$, $\int_{\Squoth} v \, d\quotprob = 0$.
  \begin{proof}
     The integral $\int_{\Squoth} v \, d\quotprob = \int_{\Squoth} \one v \, d\quotprob$ is the inner product of two elements in $L^2(\Squoth,\quotprob)$ which lie in different (orthogonal) subspaces; see \eqref{eqn:Fock-repn-of-L2(S',P)}.
  \end{proof}
\end{lemma}
Alternatively, Lemma~\ref{thm:int(u)=0-over-bdG} holds because the expectation of every odd-power monomial vanishes by \eqref{eqn:Minlos-expectation-integral}; see also \eqref{eqn:expectation-of-even-monomials} and the surrounding discussion of Remark~\ref{rem:Wiener-improves-Minlos}.

Recall that we abuse notation and write $h_x = \la h_x, \cdot \ra_\Wiener = \tilde h_x$ for elements of $\Schw'$. 

\begin{defn}\label{def:mu_x}
  Denote the measure appearing in Corollary~\ref{thm:Boundary-integral-repn-for-harm} by    
  \linenopax
  \begin{equation}\label{eqn:def:boundary-kernel}
    d\gm_x := (\one + h_x) \, d\quotprob.  
  \end{equation}
  The function \one does not show up in \eqref{eqn:integral-boundary-repn-of-h} because it is orthogonal to \Harm:
\linenopax
\begin{align*}
  \int_{\Squoth} u (\one + h_x) \, d\quotprob
  = \int_{\Squoth} u \, d\quotprob + \la u, h_x\ra_\energy
  = \la u, h_x\ra_\energy,
  \qq\text{for } u \in \Harm,
\end{align*}
where we used Lemma~\ref{thm:int(u)=0-over-bdG}. Nonetheless, its presence is necessary, %otherwise 
%\linenopax
%  \begin{align*}%\label{eqn:}
%    \int_{\Schw'} h_x \,d\quotprob 
%    = \int_{\Schw'} \one h_x \,d\quotprob 
%    = \la h_x, \one\ra_\Wiener 
%  \end{align*}
\linenopax
\begin{align*}
  \int_{\Squoth} \one d\gm_x 
  &= \int_{\Squoth} \one (\one + h_x) \, d\quotprob 
  = \int_{\Squoth} \one \, d\quotprob  + \int_{\Squoth} \one h_x \, d\quotprob 
  %= 1 + \la h_x, \one\ra_\Wiener 
  = 1,
\end{align*}
again by Lemma~\ref{thm:int(u)=0-over-bdG}. 
\end{defn}

\begin{remark}\label{rem:kernel-nonnegative}
  \version{}{\marginpar{$\gm_x \geq 0$ or $h_x \geq 0$?}}
  We have shown that as a linear functional, $\gm_x[\one]=1$. It follows by standard functional analysis that $\gm_x \geq 0$ \quotprob-a.e. on $\Squoth $. Thus, $\gm_x$ is absolutely continuous with respect to \quotprob ($\gm_x \ll \quotprob$) with Radon-Nikodym derivative $\frac{d\gm_x}{d\quotprob} = \one + h_x$.
\end{remark}

\begin{comment}
  for reasons that can best be explained in terms of the Fock space representation of $L^2(\Squot,\quotprob)$ as the second quantization of \HE: the constant function \one corresponds to the vaccuum vector; see \cite[\S4]{Hida80} for more details. It is critical to observe that $\one = 0$ in \HE, but $\one \neq 0$ on $\Schw'$.
For every $x \in \verts$, 
\end{comment}



\begin{defn}\label{def:harmonic-equivalence-of-paths}
  Recall that a path in \Graph is an infinite sequence of successively adjacent vertices. We say that a path $\cpath = (x_0, x_1, x_2, \dots)$ is a \emph{path to infinity}, and write $\cpath \to \iy$, iff \cpath eventually leaves any finite set $F \ci \verts$, i.e.,
  \linenopax
  \begin{align}\label{eqn:def:path-to-infinity}
    \exists N \text{ such that } n \geq N \implies x_n \notin F.
  \end{align}
  
  If $\cpath_1 = (x_0, x_1, x_2, \dots)$ and $\cpath_2 = (y_0, y_1, y_2, \dots)$ are two paths to infinity, define an equivalence relation by    
  \linenopax
  \begin{equation}\label{eqn:def:harmonic-equivalence-of-paths}
    \cpath_1 \simeq \cpath_2
    \q\iff\q
    \lim_{n \to \iy} (h(x_n)-h(y_n)) = 0, \q\text{for every } h \in \MP.% / \Fin.
  \end{equation}
  In particular, all paths to infinity are equivalent when $\Harm = 0$.
\end{defn}
  \glossary{name={\cpath},description={path},sort=G}

If $\gb = [\cpath]$ is any such equivalence class, pick any representative $\cpath = (x_0, x_1, x_2, \dots)$ and consider the associated sequence of measures $\{\gm_{x_n}\}$. These probability measures lie in the unit ball in the weak-$\star$ topology, so Alaoglu's theorem gives a weak-$\star$ limit
  \linenopax
  \begin{equation}\label{eqn:def:prob-meas-corr-to-a-path}
    \gn_\gb := \lim_{n \to \iy} \gm_{x_n}.% \in Prob\left(\tfrac{\Schw'}{\Fin}\right).
  \end{equation}
For any $h \in \Harm$, this measure satisfies 
  \linenopax
  \begin{equation}\label{eqn:h(xn)-becomes-h(b)}
    h(x_{n}) = \int_{\Squoth} \tilde h \,d\gm_{x_n} 
    \limas{n} \int_{\bd \Graph} \tilde h \,d\gn_\gb.
  \end{equation}
Thus, we define $\bd \Graph$ to be the collection of all such \gb, and extend harmonic functions to $\bd \Graph$ via
  \linenopax
  \begin{equation}\label{eqn:def:h(b)}
    \tilde h(\gb) := \int_{\bd \Graph} \tilde h \,d\gn_\gb.
  \end{equation}

\begin{defn}\label{def:bounded-in-HE}
  For $u \in \HE$, denote $\|u\|_\iy := \sup_{x \in \verts} |u(x)-u(o)|$, and say $u$ is \emph{bounded} iff $\|u\|_\iy < \iy$.
\end{defn}

\begin{lemma}\label{thm:Pfin-preserves-boundedness}
  If $v \in \HE$ is bounded, then $\Pfin v$ is also bounded. 
  \begin{proof}
    Choose a representative for $v$ with $0 \leq v \leq K$. Then by Corollary~\ref{thm:Boundary-integral-repn-for-harm} and \eqref{eqn:def:boundary-kernel}, 
    \linenopax
    \begin{align*}%\label{eqn:}
      \Phar v(x) = \int_{\Squoth} v(\gx) h_x(\gx) \, d\quotprob(\gx) + u(o)
           = \int_{\Squoth} v(\gx) \, d\gm_x(\gx) + u(o).
    \end{align*}
    Since $\gm_x$ is a probability measure (cf.~Remark~\ref{rem:kernel-nonnegative}), we have $\Phar v \geq 0$, and hence the finitely supported component $\Pfin v = v - \Phar v$ is also bounded. 
  \end{proof}
\end{lemma}


\begin{lemma}\label{thm:monopoles-and-dipoles-are-bounded}
  Every $v \in \MP$ is bounded. In particular, $\|v_x\|_\iy \leq R^F(o,x)$. % and $\|\monov\|_\iy = $.
  \begin{proof}
    According to Definition~\ref{def:LapM}, it suffices to check that $v_x$, \monov and \monof are bounded for each $x$. Furthermore, $\|\monof\|_\iy = \|\Pfin \monov\|_\iy \leq \|\monov\|_\iy$ by Lemma~\ref{thm:Pfin-preserves-boundedness}, and $\monov = v_x + w_o$ by definition, so it suffices to check $v_x$ and $w_o$. By \cite[Lem.~3.70]{Soardi94}, $w_o$ has a representative which is bounded, taking only values between $0$ and $w_o(o) > 0$. It remains only to check $v_x$. The following approach is taken from the ``proof'' of \cite[Conj.~3.18]{ERM}.
    
    Fix $x,y \in \verts$ and an exhaustion $\{G_k\}$, and suppose without loss of generality that $o,x,y \in G_1$. Also, let us consider the representative of $v_x$ specified by $v_x(o)=0$. On a finite network, it is well-known that 
  \linenopax
  \begin{align}\label{eqn:vx-as-prob-on-finite}
    v_x = R(o,x) u_x,  
  \end{align}
  where $u_x(y)$ is the probability that a random walker (RW) started at $y$ reaches $x$ before $o$, that is, $u_x(y) := \prob_y[\gt_x < \gt_o]$, where $\gt_x$ denotes the hitting time of $x$. This idea is discussed in \cite{DoSn84,LevPerWil08,Lyons:ProbOnTrees}. 
  
    Therefore, one can write \eqref{eqn:vx-as-prob-on-finite} on $G_k$ as $v_x^{(k)} = R_{G_k^F}(o,x) u_x^{(k)}$. In other words, $v_x^{(k)}$ is the unique solution to $\Lap v = \gd_x - \gd_o$ on the finite subnetwork $G_k^F$. Consequently, for every $k$ we have $v_x^{(k)}(y) \leq R_{G_k^F}(o,x)$ for all $y \in G_k$.
    Since $R^F(x,y) = \lim_{k \to \iy} R_{G_k^F}(x,y)$ by \cite[Def.~2.9]{ERM}, we have $\|v_x\|_\iy \leq R^F(o,x)$ for every $x \in \verts$. 
    %
  %It suffices to check this on \MP, so let $v={v_x}$ or let $v={w_x}$; recall from \cite[Lem.~2.25]{ERM} that both of these functions are bounded; they each have a representative which takes values only in $[0,1]$. 
    %Furthermore, $\|v_x\|_\energy = R(o,x)^{1/2}$ by \cite[Thm.~2.13]{ERM}, so $\left\|\frac{v_x}{\|v_x\|_\energy} \right\|_\iy = 1$. 
    %Moreover, since \Phar is a contraction, $|h({x_n})-h(o)| \leq |v(x_n) - v(o)|$, and therefore $|\gb(v)| = \lim_{n \to \iy} | \Phar v({x_n})- \Phar v(o)| \leq 1$, and \gb is bounded with $\|\gb\| \leq 1$. 
    %for any $v \in \MP$ with $\|v\|_\energy = 1$.
  \end{proof}
\end{lemma}



\begin{theorem}\label{thm:bdy-point-as-linear-fnl}
  Let $\gb \in \bd \Graph$ and let $\cpath = (x_0, x_1, x_2, \dots)$ is any representative of \gb.
  Then $\gb \in \bd \Graph$ defines a continuous linear functional on \Schw via
  \linenopax
  \begin{align}\label{eqn:bdy-pt-as-meas-limit-along-a-path}
    \gb(v) := \lim_{n \to \iy} \int_{\Schw'} \tilde v \, d\gm_{x_n}, 
    \qq v \in \Schw.
  \end{align}
  In fact, the action of \gb is equivalently given by 
  \linenopax
  \begin{align}\label{eqn:bdy-pt-as-eval-limit-along-a-path}
    \gb(v) = \lim_{n \to \iy} \Phar v({x_n})- \Phar v(o), 
    \qq v \in \Schw.
  \end{align}
  \begin{proof}
    To see that \eqref{eqn:bdy-pt-as-meas-limit-along-a-path} and \eqref{eqn:bdy-pt-as-eval-limit-along-a-path} are equivalent, compute
    \linenopax
    \begin{align*}%\label{eqn:}
      \int_{\Schw'} \cj{\tilde v} (\one + h_{x_n}) \,d\quotprob 
      = \cancel{\int_{\Schw'} \cj{\tilde v} \one \,d\quotprob} 
        + \int_{\Schw'} \cj{\tilde v} h_{x_n} \,d\quotprob 
      = \la v, h_{x_n} \ra_\energy 
      = \Phar v({x_n})-\Phar v(o),
      %\leq \|v\|_\energy \|h_x\|_\energy.
    \end{align*}
    because \one is orthogonal to \HE in $L^2(\Schw',\quotprob)$; see \eqref{eqn:Fock-repn-of-L2(S',P)}. 
       
    Now, to see that \eqref{eqn:bdy-pt-as-meas-limit-along-a-path} or \eqref{eqn:bdy-pt-as-eval-limit-along-a-path} defines a {bounded} linear functional, we only need to check that $\sup_{v \in \Schw} \{\gb(v) \suth \|v\|_\energy=1\}$ is bounded, but this is the content of Lemma~\ref{thm:monopoles-and-dipoles-are-bounded}.
    Note that the equivalence relation \eqref{eqn:def:harmonic-equivalence-of-paths} ensures that the limit is independent of the choice of representative \cpath.
  \end{proof}
\end{theorem}

\begin{remark}\label{rem:bdG-as-Diracs-at-infinity}
  In light of \eqref{eqn:bdy-pt-as-eval-limit-along-a-path}, one can think of $\gn_\gb$ in \eqref{eqn:def:prob-meas-corr-to-a-path} as a Dirac mass. Thus, $\gb \in \bd \Graph$ is a boundary point, and integrating a function $f$ against $\gn_\gb$ corresponds to evaluation of $f$ at that boundary point.
\end{remark}





